Purity in the tame cohomology

Let $(X,Z)$ be a regular pair of pure codimension $r$ over a base scheme $S$ of characteristic $p$. Under the assumption of resolution of singularities, we prove purity for the tame cohomology with coefficient in the logarithmic de Rham-Witt sheaves $\nu_m(n)$ for the regular pair $(X,Z)$, i.e. the existence of a natural isomorphism \[ Ri^!\nu_{X,m}(n)\cong \nu_{Z,m}(n-r)[-r] \] for all $m,n\geq 0$, where the logarithmic de Rham-Witt sheaves $\nu_{X,m}(n)$ are the Frobenius-fixed elements in the de Rham-Witt sheaves $W_m\Omega^{n}_{X/\mathbb{F}_p}$.

==> AcyclicityBlowUps.tex <==
% !TeX spellcheck = en_US
Let $k$ be a field. Let $X$ be a log smooth scheme over $k$, defined by a simple normal crossing divisor $D\subset X$. Let $\bar{X}\to X$ be a blowup with smooth center $Z$ and exceptional divisor $E$. Endow $\bar{X}$ with the log structure corresponding to $E\cup \bar{D}$, where $\bar{D}$ is the strict transform of $D$.  We want to compare the sheaf cohomology of $\Omega^{n,\log}_{\bar{X}}$ and  $\Omega^{n,\log}_{X}$ in good cases. We first need some lemmas describing the sheaf cohomology groups of logarithmic differentials of projective spaces. 
 
 \begin{lemma}[{\cite[Lemma 0FMH]{Stacks}}]\label{EulerSequence}
 	Let $A$ be a ring. Let $n\geq 1$ be an integer. There exists a short exact sequence
 	\begin{equation}\label{EulerSequenceSES}
 		 	0\to \Omega_{\mathbb{P}^n_A/A}\to \mathcal{O}_{\mathbb{P}^n_A}(-1)^{\oplus n+1}\to\mathcal{O}_{\mathbb{P}^n_A}\to 0. 
 	\end{equation}
 	This is called the \emph{Euler sequence}. More generally we have the sequence
 	\[
 	0\to \Omega_{\mathbb{P}^n_A/A}^j\to \bigwedge^j (\mathcal{O}_{\mathbb{P}^n_A}(-1)^{\oplus n+1})\cong \mathcal{O}_{\mathbb{P}^n_A}(-j)^{\oplus \binom{n+1}{j}}\to \Omega_{\mathbb{P}^n_A/A}^{j-1}\to 0.	
 	\]
 \end{lemma}
 Let us describe the morphisms in \eqref{EulerSequenceSES}. The sheaf \( \Omega_{\mathbb{P}^n_A/A} \) is locally generated by elements of the form
 \[
 \sum\limits_{i=0}^n f_i dX_i \quad \textrm{ such that } f_i \in \mathcal{O}_{\mathbb{P}^n_A}(-1),
 \] 
 where $X_i$ are the homogeneous coordinates of $\mathbb{P}^n_A$. The morphism on the left hand side is 
 \begin{equation}
 	\Omega_{\mathbb{P}^n_A/A}\to \mathcal{O}_{\mathbb{P}^n_A}(-1)^{\oplus n+1}=: \bigoplus_{i=0}^{n} \mathcal{O}_{\mathbb{P}^n_A}e_i, \quad
 	\sum f_idX_i\mapsto  \sum f_i e_i.
 \end{equation}	
 The right hand side is 
 \begin{equation}
	\mathcal{O}_{\mathbb{P}^n_A}(-1)^{\oplus n+1} \to \mathcal{O}_{\mathbb{P}^n_A},\quad
	\sum_{i=0}^{n}f_ie_i \mapsto  \sum_{i=0}^n f_iT_i.
 \end{equation}

Using this, we deduce the following facts on cohomology.
 \begin{lemma}[{\cite[TAG 0FUK]{Stacks}}]\label{Cohomology_of_Omega_l}
 	For any ring $A$ we have
 	\[
 	\begin{aligned}
 			&H^i(\mathbb{P}^n_A,\Omega^j_{\mathbb{P}^n_A/A})\cong 
 		\begin{cases}
 			A & \textrm{ if } 0\leq i=j\leq n\\
 			0 & \textrm{ otherwise}
 		\end{cases}\\
 	&H^i(\mathbb{P}^n_A,\Omega^j_{\mathbb{P}^n_A/A}(l))\cong 0 \textrm{ for all } l\geq 1.
 	\end{aligned}
 	\]
 \end{lemma}
 \begin{remark}\label{generatorRepresentation}
 	The sheaf cohomology groups \( H^i(\mathbb{P}^n_A,\Omega^j_{\mathbb{P}^n_A/A}) \) are isomorphic to the Čech cohomology groups \( \check{H}^i(\{U_l \to \mathbb{P}^n_A\}, \Omega^j_{\mathbb{P}^n_A/A}) \), where \( \{U_l \to \mathbb{P}^n_A\} \) is the standard affine open cover defined by \( U_l := \{X_l \neq 0\} \subseteq \mathbb{P}^n_A \).
 	
 	 The generators of $\cHH^i(\{U_l \to \mathbb{P}^n_A\},\Omega^j_{\mathbb{P}^n_A/A})$ were described in detail in \cite[TAG 0FMI]{Stacks}. A generator of $\cHH^j(\{U_l\to \mathbb{P}^n_A\},\Omega^j_{\mathbb{P}^n_A/A})$ is represented by $$(\sum_{k=0}^{j}(-1)^k\dlog(X_{i_0})\wedge \dots\widehat{\dlog X_{i_k}} \wedge \dlog(X_{i_j}))_{i_0,\dots,i_j}\in \check{C}^j(\{U_i\to \mathbb{P}^n_A\},\Omega^j_{\mathbb{P}^n_A/A}).$$
 	 
 	This can be checked inductively using the short exact sequences from \cref{EulerSequence} as follows. 
 	
 	For $j=1$, the map $\cHH^0(\mathbb{P}^n_A,\mathcal{O}_{\mathbb{P}^n_A})\to \cHH^1(\{U_l\to \mathbb{P}^n_A\},\Omega^1_{\mathbb{P}^n_A/A})$ sends $(1)_i$ to 
 	$$(dX_m/X_m-dX_n/X_n)_{mn}=(\dlog X_m-\dlog X_n)_{mn}.$$ 
 	
 	For $j\geq 1$, we consider the  general form of the Euler sequence and use the fact that the cohomology of $\mathcal{O}_{\mathbb{P}^n_A}(-1)$ vanishes. Then the image of $$\left(\sum_{k=0}^{j}(-1)^k\dlog X_{i_0}\wedge \dots\widehat{\dlog X_{i_k}} \wedge\dots \wedge \dlog X_{i_j}\right)_{i_0,\dots,i_j}\in \check{C}^j(\{U_i\to \mathbb{P}^n_A\},\Omega^j_{\mathbb{P}^n_A/A})$$
 	under the boundary morphism $H^j(\mathbb{P}^n_A,\Omega^{j}_{\mathbb{P}^n_A})\to H^{j+1}(\mathbb{P}^n_A,\Omega^{j+1}_{\mathbb{P}^n_A})$  is
 	$$(e_{i_0}/X_{i_0}\wedge \dots \wedge e_{i_j}/X_{i_j})_{i_0,\dots, i_j}\in  \check{C}^j(\{U_i\to \mathbb{P}^n_A\}, \bigwedge^{j+1} (\mathcal{O}_{\mathbb{P}^n_A}(-1)^{\oplus n+1})).$$
 	This maps to the element
 	\begin{equation*}
 			\left(\sum_{k=0}^{j+1}(-1)^k e_{i_0}/X_{i_0}\wedge \dots \wedge \widehat{e_{i_k}/X_{i_k}}\dots \wedge e_{i_{j+1}}/X_{i_{j+1}}\right)_{i_0,\dots, i_{j+1}}  
 	\end{equation*}
 	in $\check{C}^{j+1}(\{U_i\to \mathbb{P}^n_A\}, \bigwedge^{j+1} (\mathcal{O}_{\mathbb{P}^n_A}(-1)^{\oplus n+1}))$, which corresponds to 
 	\begin{equation*}
 		\left(\sum_{k=0}^{j+1}(-1)^k\dlog(X_{i_0})\wedge \dots\wedge\widehat{\dlog X_{i_k}} \wedge\dots \wedge \dlog X_{i_{j+1}}\right)_{i_0,\dots,i_{j+1}}
 	\end{equation*}
 	in $\check{C}^{j+1}(\{U_i\to \mathbb{P}^n_A\},\Omega^{j+1}_{\mathbb{P}^n_A/A}).$
 \end{remark}
 \begin{lemma}\label{1CohomologyOfLogDiffProjective}
 	Let $E$ be the projective space $\mathbb{P}^n_R$ over a regular ring $R$. Let $D=V(X_0)\subset E$ be a hyperplane divisor. Then $\Omega^n_{E/R}(\llog(D))\otimes_{\mathcal{O}_E}\mathcal{O}_E(l)$ has trivial cohomology groups for each $l\geq 0$, $n\geq 1$.  
 \end{lemma}
 \begin{proof} 
 	We may assume that $R$ is a local ring. Indeed, any cohomology group $H^i (E,\mathcal{F})$ for a coherent sheaf $\mathcal{F}$ corresponds to the global sections of the coherent sheaf $R^i\pi_*\mathcal{F}$, where $\pi$ is the projection $\mathbb{P}^n_R\to \Spec(R)$. Note that in this case $\textrm{Pic}(\mathbb{P}^n_R)=\mathbb{Z}$ and all invertible sheaves are of the form $\mathcal{O}(l)$, $l\in \mathbb{Z}$ (see \cite{Stacks}[Tag 0BXJ], note that regular local rings are UFD).\\
 	\textbf{Proof for $l=0,n=1$:}
 	
 	We have a short exact sequence of residues as in \cref{ResidueSequences}
 	\begin{equation}\label{ResidueSequenceInProof}
 		0 \to \Omega_{E/R}\to \Omega_{E/R}(\llog(D))\to \mathcal{O}_D\to 0.
 	\end{equation}

 	The cohomology group $H^i(E,\Omega_{E/R})$ and $H^i(D,\mathcal{O}_D)$ are trivial for $i\neq 1$ and $i\neq 0$ respectively by  \cref{Cohomology_of_Omega_l}.
 	
 	Now we have the long exact sequence of cohomology associated to the sequence  \eqref{ResidueSequenceInProof}
 	\begin{equation*}
		\begin{split}
			\dots &\to H^0(E,\mathcal{O}_D)\to H^1(E,\Omega_{E/R}) \\ &\to H^1(E,\Omega_{E/R}(\llog(D))) \to H^1(E,\mathcal{O}_D)= 0 \to \cdots.
		\end{split}
 	\end{equation*}		
 	We  obtain that $H^j(E,\Omega_E(\llog(D)))=0$ for all $j\geq 2$. It is left to check that the map $H^0(E,\mathcal{O}_D)\to H^1(E,\Omega_{E/R})$ is surjective. We claim that the morphism $$H^0(D,\mathcal{O}_{D})\to H^1(E,\Omega_{E/R})$$ arising from the short exact sequence is an isomorphism. For this we may instead consider \v{C}ech cohomology groups corresponding to the standard affine open covering $\{U_i=D(X_i)\}$ of $\mathbb{P}^n_R\cong E$. Now by the following diagram chase we determine the image of $1\in R\cong \cHH^0(D,\mathcal{O}_{D})$:
 	\begin{equation}\label{mainDiagramChase}
 	\resizebox{12cm}{!}{\xymatrix@C=1em{
 				&&& \cHH^0(D,\mathcal{O}_{D}) \ar[d]\\
 				& \prod_{i=0}^n\Gamma(U_i,\Omega_{E/R}) \ar[r]\ar[d]|(.3)\hole
 				& \prod_{i=0}^n\Gamma(U_i,\Omega_{E/R}(\llog(D))) \ar[r]\ar[d]|(.3)\hole
 				& \prod_{i=1}^nR[\frac{X_j}{X_i}|j=1\dots n]_0 \ar[r]\ar[d]|(.3)\hole="hole" & 0 \\
 				0\ar[r]& Z^1(E,\Omega_{E/R}) \ar[r]\ar[d] & Z^1(E,\Omega_{E/R}(\llog(D))) \ar[r] & Z^1(D,\mathcal{O}_D) \\
 				&  \cHH^1(E,\Omega_{E/R}) 
 				\ar@{<-} `l [lu]-(4,0) `"hole" `[rrruu]+(4,0) `[rruuu] [rruuu]
 				&  & \\
 				& & & 1 \ar@{|->}[d]\\
 				&0\ar@{|.>}[d]\ar@{|.>}[r] & (\dlog(X_0/X_i))_i\ar@{|->}[d]\ar@{|->}[r] & (1)_i \ar@{|.>}[d]\ar@{|.>}[r]&0,\\
 				0\ar@{|->}[r]& (\dlog(X_j)-\dlog(X_i))_{ij}\ar@{|->}[r]\ar@{|->}[d] &(\dlog(X_j)-\dlog(X_i))_{ij}\ar@{|.>}[r] &0 &\\
 				&[(\dlog(X_j)-\dlog(X_i))_{ij}]& & &
 		}}
 	\end{equation}
 	where $Z^1(E,-)$ is the kernels of the boundary morphisms 
 	\[
 	\prod\limits_{i,j=0}^n\Gamma(U_{ij},-)\to \prod\limits_{i,j,k=0}^n\Gamma(U_{ijk},-)
 	\]
 	of the \v{C}ech complex. Each of the elements 
 	$$\dlog(X_0/X_i) \in \Gamma(U_i,\Omega_{E/R}(\log(D)))$$ 
 	maps to 
 	$$1 \in \Gamma(D \cap U_i,\mathcal{O}_{D})=R[X_j|j=1,\dots,n][X_i^{-1}]_0, \quad  \textrm{ for } i>0,$$
 	 by the first residue sequence in \cref{ResidueSequences}. For $i=0$, $\dlog (X_0/X_i)=0$, but $U_0\cap D_1=\emptyset$, hence 
 	$$\Gamma(D\cap U_0, \mathcal{O}_D)\cong 0$$
 	does not contribute to the \v{C}ech cohomology group $\cHH^0(D,\mathcal{O}_{D})$.
 	
 	%correction applied, is this correct?
 	On the other hand, by \cref{generatorRepresentation}, we know that $\cHH^1(E,\Omega_{E/R})$ is generated by the class $(\dlog(X_j)-\dlog(X_i))_{ij}$.
 	
 	\textbf{Proof for $l=0, n>1$:}
 	By the second residue sequence in \cref{ResidueSequences}, we have a short exact sequence
 	\begin{equation}\label{LocalResidueSequence2}
 		0\to \Omega_{E/R}^n  \to \Omega_{E/R}^n(\llog D)\to \Omega_{D/R}^{n-1}\to 0.
 	\end{equation}
 	Note that $D$ is also a projective space isomorphic to $\mathbb{P}^{n-1}_R$. Hence 
 	\[
 	H^{j-1}(D,\Omega^{n-1}_{D/R})\cong H^{j}(E,\Omega^n_{E/R})\cong 
 	\begin{cases}
 		R &\textrm{ if }j=n\\
 		0 &\textrm{otherwise.}
 	\end{cases}
 	\]
 	We now follow the steps of \eqref{mainDiagramChase} to prove that the boundary morphism 
 	\[
 	H^{n-1}(D,\Omega^{n-1}_{D/R})\to H^{n}(E,\Omega^n_{E/R}),
 	\]
 	associated to the short exact sequence \eqref{LocalResidueSequence2}, is an isomorphism. Note that by \cref{generatorRepresentation} a generator of $$H^{n-1}(D,\Omega^{n-1}_{D/R})= \cHH^{n-1}(\{U_i\to \mathbb{P}^{n-1}_R\},\Omega^{n-1}_{\mathbb{P}^{n-1}/R})$$
 	is  
 	\begin{equation}\label{FirstValue}
 		(\sum_{k=0}^{n-1}(-1)^k\dlog(X_{i_0})\wedge \dots \wedge\widehat{\dlog X_{i_k}} \wedge\dots \wedge \dlog(X_{i_{n-1}}))_{i_0,\dots,i_{n-1}}.
 	\end{equation}
 	 Note that $i_j$ lies in $\{1,\dots n-1\}$. A preimage of \eqref{FirstValue} in $$\prod\limits_{i_0,\dots,i_{n-1}}\Gamma(U_{i_0,\dots,i_{n-1}},\Omega_{E/R}^{n}(\log(D)))$$ by the second residue sequence in \cref{ResidueSequences} is 
 	\[
 	(\sum_{k=0}^{n-1}(-1)^k\dlog(\frac{X_0}{X_{i_k}})\wedge \dlog(X_{i_0})\wedge \dots \wedge\widehat{\dlog X_{i_k}} \wedge\dots \wedge \dlog(X_{i_{n-1}}))_{i_0,\dots,i_{n-1}},
 	\]
 	as $\{\frac{X_0}{X_{i_k}}=0\}=D\cap U_{i_0,\dots,i_{n-1}}$ for any $k$ and each $U_{i_0,\dots,i_{n-1}}$. Here we allow $i_j=0$. This may be rewritten as
 	\[\begin{aligned}
		&\big(\sum_{k=0}^{n-1}(-1)^k\dlog X_{0}\wedge \dlog X_{i_0}\wedge \dots \wedge\widehat{\dlog X_{i_k}} \wedge\dots \wedge \dlog X_{i_{n-1}}\\	&-\sum_{k=0}^{n-1}\dlog X_{i_0}\wedge \dots \wedge \dlog X_{i_k} \wedge\dots \wedge \dlog X_{i_{n-1}} \big)_{i_0,\dots,i_{n-1}}.
 	\end{aligned}
 	\]
 	Finally, by straightforward computations this maps to the element
 	\[
 	(\sum_{k=0}^{n}(-1)^k\dlog X_{i_0}\wedge \dots \wedge \widehat{\dlog X_{i_k}} \wedge \dots \wedge \dlog X_{i_n})_{i_0,\dots,i_{n}}
 	\]
 	 which lies in 
 	 $$Z^n(X,\Omega_{E/R}) = \ker\left(\prod\limits_{i_0,\dots,i_n}\Gamma(U_{i_0,\dots,i_n},\Omega_{E/R})\to \prod\limits_{i_0,\dots,i_{n+1}}\Gamma(U_{i_0,\dots,i_{n+1}},\Omega_{E/R})\right),$$ 
 	 and whose class is a generator of 
 	$$H^{n}(X,\Omega^{n}_{E/R})= \cHH^{n}(\{U_i\to \mathbb{P}^{n}_R\},\Omega^{n}_{\mathbb{P}^{n}/R})$$
 	as an $R$-module by \cref{generatorRepresentation}.
 	
 	\textbf{Proof for $l\geq 1$:}	In this case the proof is simpler. We tensor the residue sequence with $\mathcal{O}_E(l)$ to obtain
 	\[
 	0\to \Omega_{E/R}^n(l)  \to \Omega_{E/R}^n(\llog D)(l)\to \Omega_{D/R}^{n-1}(l)\to 0.
 	\] 
 	We have seen in  \cref{Cohomology_of_Omega_l} that $\Omega_{E/R}^n(l)$ and $\Omega_{D/R}^{n-1}(l)$ have no higher cohomology groups since $E/R$ and $D/R$ are projective spaces. Note that tensoring $\Omega_{D/R}^{n-1}$ with $\mathcal{O}_E(l)$ corresponds to tensoring with $\mathcal{O}_D(l)$, thereby concluding that $\Omega_{E/R}^n(\llog D)(l)$ has no higher cohomology groups.
 \end{proof}

 \begin{proposition}[\cite[Theorem 6.1]{KelleyCohomology}] \label{AcyclicityProposition}
 		Let $k$ be a perfect field of positive characteristic.
 		Let $X=\Spec(A)$ be a connected affine log smooth log scheme over $k$ whose log structure is defined by a normal crossing divisor $D\subset X$. Let $f:\bar{X}\to X=\Spec(A)$ be a blowup in a smooth center $Z\subset D$, such that the exceptional divisor $E$ intersects the strict transform $\bar{D}$ of the divisor $D$ transversally. Then \[H^i(\bar{X},\Omega^{n}_{\bar{X}/k}(\llog(E+\bar{D})))=0 \quad  \textrm{for } \quad i>0, n\geq 0.\]
 \end{proposition}

%  		We prove the theorem by induction on $n$. For $n=0$, $\Omega^{n}_{\bar{X}/k}(\llog D)=\mathcal{O}_{\bar{X}}$. This case is proven by Chatzistamatiou and Rülling in  \cite[Theorem 1.1]{CR15} . Let $n\geq 1$.
 		
%  	 	Note that $R^if_*\Omega^{n,\llog}_{\bar{X}}$ is a coherent sheaf, as $\Omega^n_{\bar{X},\llog}$ is also coherent and $f$ is proper \cite[TAG 02O4]{Stacks}. Hence $R^if_*\Omega^{n,\llog}_{\bar{X}}$ is the coherent sheaf corresponding to the $A$-module  $H^i(\bar{X},\Omega^{n,\llog}_{\bar{X}})$. 
 	 	
%  	 	\textbf{Reduction Step 1:} 
%  	 	We first reduce to the case when $D$ is a regular irreducible divisor containing $Z$:
 	 	
%  	 	Write $D=D_1\cup \dots \cup D_n$, where $D_i$ are the irreducible components of $D$. Write $\bar{D}=\bar{D}_1\cup \dots \cup\bar{D}_n$, where each $\bar{D}_i$ is the strict transform of $D_i$. Since $Z$ is smooth and connected, we may assume that it is contained in a single $D_i$, say $D_1$. We also define $\tilde{D}:=\bar{D}\cap E$.
 	 	
%  	 	The second residue sequence in \cref{ResidueSequences} states that 
%  	 	\begin{equation}
%  	 		0\to \Omega^{n}_{\bar{X}/S}(\llog(E+\bar{D}-\bar{D}_i))\to \Omega^n_{\bar{X}/S}(\llog(E+\bar{D}))\to \Omega_{\bar{D_1}/S}^{n-1}(\llog(E+\bar{D}-\bar{D}_i)|_{\bar{D}_i})\to 0
%  	 	\end{equation}
%  	 	is exact. By induction on the number of divisors $D_i\neq D_1$, we reduce to the case where $D=D_1$ as follows:
 	 	
%  	 	$Z\cap D_i$ is contained in $D_1\cap D_i$, which allows us to use the induction step on $n$ by applying theorem \cr{AcyclicityProposition} to $\Omega^{n-1}_{\bar{D}_i/S}(\llog(E+\bar{D}-\bar{D}_i)|_{\bar{D}_i})$. Thus by the long exact sequence of cohomology we obtain
%  	 	\[\begin{aligned}
%  	 		&\dots \to H^1\big(\bar{X},\Omega^n_{\bar{X}/S}(\llog(E+\bar{D}-\bar{D}_i))\big)\to H^1\big(\bar{X},\Omega^n_{\bar{X}/S}(\llog(E+\bar{D}))\big)\to\\ &H^1\big(\bar{D}_i,\Omega^{n-1}_{\bar{D}_i/S}(E+\bar{D}-\bar{D}_i )|_{\bar{D}_i}\big)\cong 0\to \dots\to
%  	 		H^j\big(\bar{X},\Omega^n_{\bar{X}/S}(\llog(E+\bar{D}-\bar{D}_i))\big)\\\
%  	 		&\to H^j\big(\bar{X},\Omega^n_{\bar{X}/S}(\llog(E+\bar{D}))\big)\to H^j\big(\bar{D}_i,\Omega^{n-1}_{\bar{D}_i/S}(E+\bar{D}-\bar{D}_i)|_{\bar{D}_i}\big)\cong 0\to \dots.
%  	 	\end{aligned}
%  	 	\] 
%  	 	Hence $H^1\big(\bar{X},\Omega^n_{\bar{X}/S}(\llog(E+\bar{D}-\bar{D}_i))\big)\to H^1\big(\bar{X},\Omega^n_{\bar{X}/S}(\llog(E+\bar{D}))\big)$ is surjective and $H^j\big(\bar{X},\Omega^n_{\bar{X}/S}(\llog(E+\bar{D}-\bar{D}_i))\big)\to H^j\big(\bar{X},\Omega^n_{\bar{X}/S}(E+\bar{D})\big)$ is an isomorphism for $j\geq 2$. Note here that it was essential not to remove the divisor $D_1$. Otherwise, one can not apply the induction step of the theorem on $D_i$.
 	 	
%  	 	\textbf{Reduction Step 2:} 
%  	 	Zariski-locally, $Z$ is a complete intersection in $X$, defined by $(f_1,\dots,f_c)$, where $c=\textrm{codim}_X(Z)$. We may furthermore assume that $D=V(f_1)$:
 	 	
%  	 	 Indeed, let $x\in X$ be a closed point. Then $\mathcal{I}_Z/\mathfrak{m}_x\mathcal{I}_{Z}$ has a basis defined by $(\bar{f}_1,\dots,\bar{f}_c)$. Let $\alpha$ be a generator of $\mathcal{I}_{D,x}$ as an $\mathcal{O}_{X,x}$-module. Then $\bar{\alpha}$ lies in $\mathcal{I}_Z/\mathfrak{m}_x\mathcal{I}_Z$ and is nonzero. In particular we may replace one of the basis elements, say $\bar{f}_1$ by $\bar{\alpha}$. By Nakayama, $(\bar{f}_1,\dots,\bar{f}_n)$  lift to  a set of minimal generators $(f_1,\dots, f_c)$ of $\mathcal{I}_{Z,x}$. We may then find an affine open $U$ of $X$ containing $x$, for which $(f_1,\dots,f_c)$ generate $\mathcal{I}_Z$ since $\mathcal{I}_Z$ is coherent.
 	 	
%  	 	We can now describe the inclusion $\tilde{D}=E\cap \bar{D}\to E$. We have $$\tilde{D}=\textrm{Proj}(\bigoplus_{n=1}^\infty (I_{Z}/f_1)^n/(I_Z/f_1)^{n+1}) \cong \textrm{Proj}(A/I_Z[X_2,\dots X_c])\cong \mathbb{P}_Z^{c-2}$$
%  	 	and 
%  	 	$$ E=\textrm{Proj}(\bigoplus_{i=1}^\infty I_{Z}^n/I_Z^{n+1}) \cong \textrm{Proj}(A/I_Z[X_1,\dots X_c])\cong \mathbb{P}_Z^{c-1},$$	
%  	 	where $\tilde{D}$ corresponds to $V(X_1)$ in $\mathbb{P}^{c-1}_Z\cong E$. 
 	 	
%  		\textbf{Reduction Step 3:} We reduce the problem to computing sheaf cohomology groups of the projective space $E=\mathbb{P}^{c-1}_Z$:
 		
%  	 	To prove the claim we only need to check that $(R^if_*\Omega^{n,\llog}_{\bar{X}})_x$ is zero at every point $x\in \Spec(A)$.
 	 	
%  	 	The scheme $V:=X\backslash Z$ is isomorphic to $\bar{X}\backslash E$. We can then cover $V$ by affine opens $V_i$ for which $H^i(V_i,\Omega^{n,\llog}_{\bar{X}})=0$ as $\Omega^{n,\llog}_{\bar{X}}$ is coherent. Hence $(R^if_*\Omega^{n,\llog}_{\bar{X}})_x$ is zero at every point $x\in V$. 
 	 	
%  	 	It remains to check that  $(R^if_*\Omega^{n,\llog}_{\bar{X}})_x$ is zero at each point $x\in Z$. This group is isomorphic to $H^i(\bar{X},\Omega^{n,\llog}_{\bar{X}})\otimes_AA_{\mathfrak{p}}$, where $\mathfrak{p}$ is the prime ideal of $A$ associated to $x$. The theorem on formal functions \cite{Stacks}[TAG 02OC] states that 
%  	 	$$H^i(\bar{X},\Omega^{n,\llog}_{\bar{X}})\otimes_A \hat{A}\cong \textrm{colim}_lH^i(E,\Omega^{n,\llog}_{\bar{X}}\otimes_{\mathcal{O}_{\bar{X}}} \mathcal{O}_{\bar{X}}/\mathcal{I}_E^l),$$
%  	 	where $\hat{A}$ is the completion of $A$ with respect to the ideal $I_E$ cutting out $E$.
%  	 	Since $A_{\mathfrak{p}}\to \hat{A}_{\mathfrak{p}}\cong \hat{A}\otimes_AA_{\mathfrak{p}}$ is faithfully flat \cite[TAG 00MO]{Stacks}, $H^i(\bar{X},\Omega^{n,\llog}_{\bar{X}})\otimes_AA_{\mathfrak{p}}$ is trivial if the same holds for $H^i(\bar{X},\Omega^{n,\llog}_{\bar{X}})\otimes_A\hat{A}_{\mathfrak{p}}=H^i(\bar{X},\Omega^{n,\llog}_{\bar{X}})\otimes_A\hat{A}\otimes_A A_{\mathfrak{p}}$. It then suffices to check that $H^i(E,\Omega^{n,\llog}_{\bar{X}}\otimes_{\mathcal{O}_{\bar{X}}} \mathcal{O}_{\bar{X}}/\mathcal{I}_E^l)$ is trivial. We prove this by induction on $l$.\\
  	 	
%   	 	\textbf{Computations:}
 	 	  
%  	 	\textbf{Case $l=1$:} \quad  Let $\iota_E:E\to \bar{X}$ be the natural inclusion. We investigate $$\Omega^{n,\log}_{\bar{X}}\otimes_{\mathcal{O}_{\bar{X}}}\mathcal{O}_E=\iota_{E,*}\Omega^{n,\llog}_{\bar{X}}.$$
 	 	
%  	 	The blowup centre $Z$ is smooth, hence $E$ is irreducible (we already showed that $E\cong \mathbb{P}_Z^{c-1})$). Therefore $E$ is defined by cutting out an ideal in $\mathcal{O}_{\bar{X}}$ generated by the coherent monoidal ideal $\mathcal{I}_E\cap \mathcal{M}_{\bar{X}}$ in $\mathcal{M}_{\bar{X}}$ which is locally the logification of the monoid $\iota_{E,*}\mathbb{N}$. By Lemma \cr{PullbackOfLogDiff}
%  	 	  \[
%  	 	  \Omega^{\log}_{\bar{X}/S}\otimes_{\mathcal{O}_{\bar{X}}}\mathcal{O}_E\cong \Omega^{\log}_{E/S},
%  	 	  \]
%  	 	  where we endow $E$ with the log structure inherited from $\bar{X}$. By Corollary \cr{ShortExactSequencePullBack} we have a short exact sequence
%  	 	  \begin{equation}\label{StarSequence}
%  	 	  	0\to \Omega_{E/S}^{n}(\llog \tilde{D})\to \Omega_{E/S}^{n,\log} \to \Omega_{E/S}^{n-1}(\llog \tilde{D})\to 0.
%  	 	  \end{equation}
%  	 	  Hence, it suffices to check that the higher cohomology groups of $\Omega_{E/S}^n(\llog\tilde{D})$ are trivial for each $n\geq 0$. Since $Z$ is smooth, locally on $X$, $\Omega_{Z/S}$ is free \cite[TAG 02G1]{Stacks}. After localization of $X$, the fundamental exact sequence takes the form
%  	 	  \[
%  	 	  0\to \Omega_{Z/S}\otimes \mathcal{O}_E\cong \mathcal{O}_E^{\oplus m}\to \Omega_{E/S}(\llog \tilde{D})\to \Omega_{E/Z}(\llog \tilde{D})\to 0.
%  	 	  \]
%  	 	  where $m=\dim Z$. Note that the map on the LHS is injective since $E\to Z$ is log smooth. We obtain by Lemma \cr{twoStepFiltration} below a filtration 
%  	 	  \[
%  	 	  0=F_0\subseteq F_1 \subseteq \dots \subseteq F_{n}\subseteq F_{n+1}:= \Omega_{E/S}^n(\llog \tilde{D})
%  	 	  \]
%  	 	  such that 
%  	 	  $$F_{i+1}/F_{i}\cong \bigwedge^{n-i}\mathcal{O}_E^{\oplus m}\otimes\Omega_{E/Z}^{i}(\llog \bar{D}).$$
%  	 	  The module $F_{i+1}/F_{i}$ is then a direct sum of copies of $\Omega_{E/Z}^{i}(\llog \bar{D})$, whose higher cohomology vanishes for every $i\geq 1$ by Lemma \cr{1CohomologyOfLogDiffProjective}. For $i=0$, $\Omega^0_{E/Z}(\log \tilde{D})=\mathcal{O}_E$. Its cohomology groups vanish by 
 	 	  
%  	 	  \textbf{Case $l>1$:}\quad  We prove this part using induction on $l$. We have the short exact sequence 
%  	 	  \[
%  	 	  0\to \Omega^{n,\log}_{\bar{X}/S}\otimes_{\mathcal{O}_{\bar{X}}}\mathcal{I}_E^{l}/\mathcal{I}_E^{l+1}\to \Omega_{\bar{X}/S}^{n,\llog}\otimes_{\mathcal{O}_{\bar{X}}}\mathcal{O}_{\bar{X}}/\mathcal{I}_E^{l+1} \to \Omega^{n,\llog}_{\bar{X}/S}\otimes_{\mathcal{O}_{\bar{X}}}\mathcal{O}_{\bar{X}}/\mathcal{I}_E^{l}\to 0.
%  	 	  \]
%  	 	  Note that $\mathcal{I}_E^{l}/\mathcal{I}_E^{l+1} \cong \mathcal{O}_E(l)$. Therefore we have to prove that 
%  	 	  \[
%  	 	  \Omega_{E/S}^{n,\log}\otimes_{\mathcal{O}_E}\mathcal{O}_E(l)=:\Omega_{E/S}^{n,\log}(l)
%  	 	  \]
%  	 	  has no higher cohomology. Tensoring sequence (\cr{StarSequence}) with $\mathcal{O}_E(l)$ reduces to proving that $\Omega_{E/Z}^i(\llog \tilde{D})(l)$ has no higher cohomology, which is the case by Lemma \cr{1CohomologyOfLogDiffProjective}.
% \end{proof}
% \begin{remark}
% 	I was notified by A. Merici that a proof of Theorem \cr{AcyclicityProposition} has been given in \cite[Theorem 6.1]{KelleyCohomology} and is also a special case of Theorem 5.2. of \cite{SaitoReciprocity}.
% \end{remark}


% \subsubsection*{Technicalities about wedge products}
% The next lemma is essential for studying the cohomology of wedge products of locally free sheaves. It is often used in the literature, however with no proof that I found.
% \begin{lemma}\label{twoStepFiltration}[two step filtration, folklore]
% 	Let $(X,\mathcal{O}_X)$ be a locally ringed space. Let 
% 	\[
% 	0\to \mathcal{U}\to\mathcal{V}\xrightarrow{g} \mathcal{W}\to 0
% 	\]
% 	be a short exact sequence of locally free sheaves. Then there is for every $k\in \mathbb{N}$ a filtration
% 	\[
% 	0=\mathcal{F}_0\subseteq \mathcal{F}_1\subseteq \cdots \subseteq \mathcal{F}_k\subseteq \mathcal{F}_{k}\subseteq \mathcal{F}_{k+1}=\bigwedge^k\mathcal{V}
% 	\]
% 	such that 
% 	\[
% 	\mathcal{F}_{i+1}/\mathcal{F}_i\cong \bigwedge^{k-i}\mathcal{U}\otimes_{\mathcal{O}_X}\bigwedge^i\mathcal{W}.
% 	\]
% \end{lemma}
% \begin{proof}
% 	Define $\mathcal{F}_i$ as the  subsheaf of $\bigwedge^k\mathcal{V}$ generated locally by 
% 	\[
% 	u_1 \wedge \dots \wedge u_{k+1-i}\wedge v_1 \wedge \dots \wedge v_{i-1} 
% 	\]
% 	where each $u_j$ is a section of $\mathcal{U}$ and each $v_j$ is a section of $\mathcal{V}$. 
% 	The isomorphism 
% 	\[
% 	\mathcal{F}_{i+1}/\mathcal{F}_i\xrightarrow{\phi} \bigwedge^{k-i}\mathcal{U}\otimes_{\mathcal{O}_X}\bigwedge^i\mathcal{W},
% 	\]
% 	is defined by
% 	\[
% 	u_1 \wedge \dots \wedge u_{k-i}\wedge v_1 \wedge \dots \wedge v_{i} \mapsto u_1 \wedge \dots \wedge u_{k-i}\otimes g(v_1)\wedge \dots \wedge g(v_{i}). 
% 	\]
% 	We now prove that this is an isomorphism. Arguing locally , we need to prove that the claim holds when $\mathcal{U}$, $\mathcal{V}$ and $\mathcal{W}$ are free modules over  a local ring $A$. By Nakayama's lemma $\mathcal{V}$ has a basis $v_1, \dots , v_m$ where $m=\textrm{rank}(\mathcal{V})$, such that $v_1,\dots v_l$ is a basis of $\mathcal{U}$  where $l=\textrm{rank}(\mathcal{U})$. Therefore $\mathcal{F}_{i+1}$ has a basis consisting of  $v_{i_1}\wedge \dots\wedge v_{i_k}$ where $i_1<\dots <i_k$ and $i_1,\dots i_{k-i}\leq l$. The latter has a basis of $\mathcal{F}_i$ of the same form as a subbasis. Hence $\mathcal{F}_{i+1}/\mathcal{F}_i$ has a basis generated by classes of $v_{i_1}\wedge \dots \wedge v_{i_k}$ such that $i_1< \dots <i_{k-i}\leq l <i_{k-i+1} <\dots <i_k$. On the other hand 
% 	\[
% 	\bigwedge^{k-i} \mathcal{U}\otimes_A\bigwedge^{i}\mathcal{W}
% 	\]
% 	has a basis generated by $v_{i_1}\wedge \dots \wedge v_{i_{k-i}}\otimes g(v_{i_{k-i+1}}) \wedge \dots \wedge g(v_{i_{k}})$ where $i_1< \dots< i_{k-i} \leq l<i_ {k-i+1}<\dots <i_k$. Since $\phi$ sends the basis elements of $\mathcal{F}_{i+1}/\mathcal{F}_i$ to the respective basis elements of $\bigwedge^{k-i} \mathcal{U}\bigotimes_A\bigwedge^{i}\mathcal{W}$, we obtain an isomorphism.
% \end{proof}
% We get the evident corollaries
% \begin{corollary}
% 	In the case of the previous corollary, if $\mathcal{U}$ is of rank $1$ then
% 	\[
% 	0\to \mathcal{U}\otimes \bigwedge^{k-1}\mathcal{W}\to \bigwedge^k\mathcal{V}\to \bigwedge^k  \mathcal{W}\to 0,
% 	\]
% 	is exact. If $\mathcal{W}$ is of rank $1$ then
% 	\[
% 	0\to \bigwedge^k \mathcal{U}\to \bigwedge^k\mathcal{V}\to \bigwedge^{k-1}\mathcal{U}\otimes \mathcal{W}\to 0
% 	\]
% 	is exact.
% \end{corollary}
% %\begin{remark}
% %	\cref{AcyclicityProposition} is \'etale-local on $X$.
% %\end{remark}
% %\begin{proof}
% %	First, note that the claim is  Zariski-local on $X$. 
% %	
% %	Let $Y\to X$ be an \'etale morphism. Denote by $\bar{Y}$ and $\bar{X}$ the blowups of $Y$ and $X$ in $Z\times_XY:=Z_Y$ and $Z$ respectively. We know (see \cite{Stacks}[TAG 0805])that blow-ups commute with flat morphisms, i.e. the diagram 
% %	\[\centering
% %	\begin{tikzcd}
% %		\bar{Y} \ar[r,"\pi_Y"] \ar[d,"\bar{f}"] &Y \ar[d,"f"]\\
% %		\bar{X} \ar[r, "\pi_X"] & X
% %	\end{tikzcd}
% %	\]
% %	is Cartesian.
% %	
% %	The scheme $Y$ can be endowed with the log structure associated to the divisor $D_Y$ which is the pullback of $D$ via $Y\to X$, \cite{Stacks}[TAG 02OO].  Since $\bar{f}:\bar{Y}\to \bar{X}$ is \'etale, we have $\bar{f}^*\Omega_{\bar{X}/S,\llog}\cong \Omega_{\bar{Y}/S,\llog}$. We may therefore use flat base change \cite{Stacks}[tag 02KH], stating that the base change morphism
% %	\[
% %	f^* R^i\pi_{X,*} \Omega_{\bar{X}/S,\llog}\to R^i\pi_{Y,*} \bar{f}^*\Omega_{\bar{X}/S,\llog} \cong 	R^i\pi_{Y,*} \Omega_{\bar{Y}/S,\llog}
% %	\]
% %	is an isomorphism.  
% %	We conclude that $R^i\pi_{X,*}\Omega_{\Bar{X}/S,\llog}$ is trivial if and only if for every \'etale covering  $\{Y_j\to X\}$ of $X$, the sheaf $R^i\pi_{Y_j,*}\Omega_{\bar{Y}_j/S,\llog}$ is trivial.
% %\end{proof}
